Scientific Hypothesis Generation and Validation: Methods, Datasets, and Future Directions

Large Language Models (LLMs) are transforming scientific hypothesis generation and validation by enabling information synthesis, latent relationship discovery, and reasoning augmentation. This survey provides a structured overview of LLM-driven approaches, including symbolic frameworks, generative models, hybrid systems, and multi-agent architectures. We examine techniques such as retrieval-augmented generation, knowledge-graph completion, simulation, causal inference, and tool-assisted reasoning, highlighting trade-offs in interpretability, novelty, and domain alignment. We contrast early symbolic discovery systems (e.g., BACON, KEKADA) with modern LLM pipelines that leverage in-context learning and domain adaptation via fine-tuning, retrieval, and symbolic grounding. For validation, we review simulation, human-AI collaboration, causal modeling, and uncertainty quantification, emphasizing iterative assessment in open-world contexts. The survey maps datasets across biomedicine, materials science, environmental science, and social science, introducing new resources like AHTech and CSKG-600. Finally, we outline a roadmap emphasizing novelty-aware generation, multimodal-symbolic integration, human-in-the-loop systems, and ethical safeguards, positioning LLMs as agents for principled, scalable scientific discovery.

==> Sections/0_abstract.tex <==
\begin{abstract}

Large Language Models (LLMs) have emerged as transformative tools in scientific hypothesis creation and validation, offering capabilities to synthesize vast information, extract latent relationships, and augment human reasoning. This survey provides a structured and comprehensive overview of LLM-based approaches across both hypothesis generation and validation pipelines. We categorize these approaches into symbolic frameworks, generative models, hybrid systems, and multi-agent architectures, highlighting methodologies such as knowledge-graph completion, retrieval-augmented generation, simulation-based exploration, causal inference, and tool-augmented reasoning. We analyze their strengths, limitations, and the trade-offs between interpretability, novelty, and domain alignment.
We further examine computational frameworks for discovery, including early symbolic systems like BACON and KEKADA, contrasting them with modern LLM pipelines that define and traverse complex hypothesis spaces through in-context learning and generative prompting. A special focus is given to domain knowledge integration, with techniques such as fine-tuning, retrieval augmentation, tool use, and symbolic-scientific reasoning enabling LLMs to specialize in high-stakes, domain-specific contexts. In hypothesis validation, we analyze simulation-based testing, human-AI collaborative filtering, multimodal verification, causal modeling, and uncertainty quantification, and we emphasize the importance of iterative validation, especially in open-world and high-risk domains.
The survey systematically reviews diverse datasets across biomedicine, materials science, environmental research, and the social sciences, characterizing them by modality, evaluation criteria, feasibility for generative reasoning, and limitations in novelty or bias. We introduce new entries such as the AHTech electrolyte additive library and CSKG-600 for knowledge-graph-based evaluation and map datasets to modeling modalities such as text, tabular, molecular, and multi-omics.
Finally, we propose a forward-looking roadmap: generative exploration with novelty-aware objectives, multimodal grounding and symbolic reasoning, human-in-the-loop frameworks, and cross-domain knowledge transfer. We advocate for new metrics that assess correctness, plausibility, novelty, and risk, and we underscore the need for principled ethical safeguards in hypothesis generation. Through these directions, LLMs can evolve from language tools into scientifically grounded agents capable of steering discovery, mitigating risk, and shaping a new paradigm of machine-augmented scientific reasoning.

\end{abstract}
